Unmanned Aerial Vehicles in Logistics: Efficiency Gains and Communication Performance of Hybrid Combinations of Ground and Aerial Vehicles

Unmanned Aerial Vehicles (UAVs) have drastically gained popularity in various Intelligent Transportation System (ITS) applications to improve the safety and efficiency of transportation systems. In this context, the combination of ground vehicles, such as delivery trucks, with drones to assist in the last mile pick-up and delivery of the parcels has been recently proposed. While aerial vehicles promise increased efficiency based on flexible routes and parallelized operation, highly reliable wireless communication is also required for the control and coordination of potentially many drones acting in a self-organized way. In this paper, we analyze the improvements procured by drone usage in parcel delivery compared to traditional delivery and propose a simulation framework to further quantify the efficiency gains of the parcel delivery logistics and to analyze the performance of different wireless communications options. To this end, we consider a heterogeneous vehicle routing problem with various constraints. We consider two approaches regarding the dispatching and recovery of drones and evaluate their benefits as opposed to parcel delivery with a classic truck only. Furthermore, we compare two networking technologies for enabling coordination of the self-organizing teams of drones with a realistically modeled environment: one approach relying on base station oriented Long Term Evolution (LTE) vs. a more decentralized Cellular Vehicle-to-Everything (C-V2X) solution. The results show time savings of nearly 40% can be achieved through drone usage and that the negative impact of urban shadowing on network communications in the base station oriented LTE approach can be compensated by leveraging decentralized C-V2X communications

==> tex/tables/energy-evaluation-parameters.tex <==
%\newcommand{\entry}[2]{#1 & #2 \\}
%\newcommand{\head}[2]{\toprule \entry{\textbf{#1}}{\textbf{#2}}\midrule}
%
%\newcommand{\sideHeader}[3]
%{
%	\multirow{#1}{*}{
%		\rotatebox[origin=c]{90}{
%			\parbox{#2}{\centering \textbf{#3}}
%		}
%	}
%}

\begin{table}[ht]
	\centering
	\caption{Parameters of energy savings evaluation}
	\begin{tabular}{ll}
%		\sideHeader{13}{0.5cm}{General} 
		\head{Parameter}{Value}
%		\entry{\textbf{Parameter}}{\textbf{Value}}
		
		\entry{Simulation duration}{until delivery completion}
		\entry{Runs per configuration}{10}
		\entry{Scenario size}{3000~m x 1500~m x 250~m}

		\entry{Maximum speed (Truck)}{...}
		\entry{Maximum speed (UAV)}{16~mps}
		\entry{Number of deliveries}{10,~15,~20}
		\entry{UAV count}{\{0,~1,~2,~3\}}

	
		\bottomrule
		
	\end{tabular}
	\label{tab:energy-evaluation-parameters}
\end{table}

